Model Predictive Contouring Control for Collision Avoidance in Unstructured Dynamic Environments

This paper presents a method for local motion planning in unstructured environments with static and moving obstacles, such as humans. Given a reference path and speed, our optimization-based receding-horizon approach computes a local trajectory that minimizes the tracking error while avoiding obstacles. We build on nonlinear model-predictive contouring control (MPCC) and extend it to incorporate a static map by computing, online, a set of convex regions in free space. We model moving obstacles as ellipsoids and provide a correct bound to approximate the collision region, given by the Minkowsky sum of an ellipse and a circle. Our framework is agnostic to the robot model. We present experimental results with a mobile robot navigating in indoor environments populated with humans. Our method is executed fully onboard without the need of external support and can be applied to other robot morphologies such as autonomous cars.

==> eqs_for_images.tex <==
\begin{align*}
X\\
Y\\
e_k^l\\
e_k^c\\
\phi^{\boldsymbol{p}}(\theta_k)\\
\tilde{e}^c(\boldsymbol{z}_k,\theta_k)\\
\tilde{e}^l(\boldsymbol{z}_k,\theta_k)\\
[x_k,y_k,\phi _k]\\	
[x_{m-1}^p,y_{m-1}^p]\\	
[x_m^p,y_m^p]\\				%% Yet to replace in image!
[x_{m+1}^p,y_{m+1}^p]\\  	%% Yet to replace in image!
[x_{m+2}^p,y_{m+2}^p]\\		%% Yet to teplace in image!
[x^{r}(\theta),y^{r}(\theta)]\\
[x^{r}(\theta_k),y^{r}(\theta_k)]\\
s_m\\
\theta
\end{align*}

\begin{align*}
v_B\\
v_{A_i}\\
-v_{A_i}\\
v_{B_1,A_i}\\
v_{B_2,A_i}\\
r_{A_i}\\
r_B\\
B\\
A_i\\
r_{A_i} + r_B\\
\hat{B}_1\\				%% Yet to replace in image!
\hat{B}_2\\				%% Yet to replace in image!
\hat{A}_i\\				%% Yet to replace in image!
\lambda_{r_1}\\
\lambda_{r_2}\\
\lambda_{f_1}\\
\lambda_{f_2}\\
\lambda_{B_1A_i}\\
\lambda_{B_2A_i}\\
\end{align*}

\begin{align*}
a\\
b\\
v_{x,k}\\
v_{y,k}\\
r_{\textrm{disc}}\\
\Delta_{x,k}\\
\Delta_{y,k}\\
\Delta x^{1}_{k}\\
\Delta y^{1}_{k}\\
\Delta x^{2}_{k}\\
\Delta y^{2}_{k}
\end{align*}

\begin{align*}
    r_c\\
    r_N\\
    r_0\\
    r_{m + 1}\\
    r_{m + 2}\\
    \psi
\end{align*}

$$\pazocal{P}$$

$$\pazocal{O}^{\text{static}},\, \pazocal{O}^{\text{dynamic}}$$

==> minimum_bound.tex <==
\subsubsection{Minimum bound}

The parametric equation defining the Minkowski Sum of an ellipsoid with a circle is:

\begin{equation}
    \right[
    \begin{bmatrix}
    x = a+\frac{b r}{\sqrt[b^2\cos{\theta}^2 + a^2\sin{\theta}^2])}}\\
    y = b + \frac{a r}{\sqrt{b^2\cos{\theta}^2 + a^2\sin{\theta}^2}}
    \end{bmatrix}
    \left]
\end{equation}

According with the theorem proposed by \cite{uteshev2015metric} the minimum distance between two quadratic shapes is the minimal positive zero of the polynomial:

\begin{equation}\label{eq:minimum_polynom}
    F(z) = D_\lambda(\det{\lambda*E_1+(z-\lambda E_2)-\lambda(z-\lambda E_1E_2)})
\end{equation}

provided that this zero is not a multiple one. Here ${\mathcal{D}_{\lambda}$ stands for the discriminant of the polynomial treated w.r.t. $\lambda$

We use a determinantal representation of the discriminant as defined in cite. The minimum distance equation can be used to compute the minimum dimensions of an ellipsoid which bounds the Minkowski Sum of an ellipsoid with a circle. Consider the ellipsoid $E_1$ and $E_2$ as follows:

\begin{equation}
    E_1 = x^T\begin{bmatrix}
       \frac{1}{(a+\delta)^2} &  0           \\[0.3em]
       0 & \frac{1}{(b+\delta)^2} \\[0.3em]
     \end{bmatrix}x
\end{equation}

\begin{equation}
    E_2 = x^T\begin{bmatrix}
       \frac{1}{(a)^2} &  0           \\[0.3em]
       0 & \frac{1}{(b)^2} \\[0.3em]
     \end{bmatrix}x
\end{equation}

with $a$ and $b$ as the semi-major and semi-minor of ellipsoid $E_2$ respectively, and $\delta$ is an enlargement distance of ellipsoid $E_1$ with respect to $E_2$.
The \cref{eq:minimum_polynom} can now be used to obtain the minimum distance between $E_1$ and $E_2$ resulting in the following equation:

\begin{equation}
    Dist_{min}=\frac{4 a b \delta^2 + 2 a \delta^3 + 2 b \delta^3}{a^2 + 2 a b + b^2 + 2 a \delta + 2 b \delta}
\end{equation}

In order to find the bounding ellipsoid it is necessary to find the value of $\delta$ such that $Dist_min \ge r$. with $r$ as the radius of the circle. The solution can be found numerically in the positive neighborhood of zero. A close formula can also be obtained but due to its extension it is not presented in this paper. The resulting bounding ellipse and shape of the Minkowski Sum can be observed in \cref{.}

\begin{theorem}
Let $E_1$ and $E_2$ be a function whose derivative exists in every point, then $f$ 
is a continuous function.
\end{theorem}

==> sec/backup.tex <==
\begin{table*}[]
        \caption{Computation times of the proposed algorithm. \todo{Solver times on the left in bold and computation of collision free area on the right in [ms]}\LF{Can we write the total time (i.e., solver times and computation collision free area) and add between brackets the time needed for the computation of the collision free area? I would remove the min values to make it more compact}.}
        \centering
        \begin{tabular}{|l|llll|llll|llll|}
        \hline
        \multirow{2}{*}{\diagbox{Velocity [m/s]}{$T_{\textrm{horizon}}$ [s]}} & \multicolumn{4}{c|}{1}                                                                                                      & \multicolumn{4}{c|}{3}                                                                                                     & \multicolumn{4}{c|}{5}                                                                                                       \\ \cline{2-13} 
                                   & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Min.} & \multicolumn{1}{c}{Max.} & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Min.} & \multicolumn{1}{c}{Max.} & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Min.} & \multicolumn{1}{c}{Max.} & \multicolumn{1}{c|}{$\sigma$} \\ \hline
        1                  & \textbf{15} / 28                           & \textbf{1.5} / 1.9                       & \textbf{34.9} / 35.15                        & \textbf{6.7} / 32.5                               & \textbf{15} / 28                           & \textbf{15} / 28                       & \textbf{15} / 28                         & \textbf{15} / 28                               & \textbf{15} / 28                           & \textbf{15} / 28                       & \textbf{15} / 28                         & \textbf{15} / 28                               \\ \hline
        1.25            & \textbf{8.3} / 19.7                           & \textbf{15} / 28                       & \textbf{15} / 28                         & \textbf{15} / 28                               & \textbf{15} / 28                           & \textbf{15} / 28                       &\textbf{15} / 28                         & \textbf{15} / 28                               & \textbf{15} / 28                           & \textbf{15} / 28                       & \textbf{15} / 28                        & \textbf{15} / 28                               \\ \hline
        1.5          & \textbf{7.2} / 16.9                              & \textbf{15} / 28                          & \textbf{15} / 28                            & \textbf{15} / 28                              & \textbf{15} / 28                          & \textbf{15} / 28                       & \textbf{15} / 28                         & \textbf{15} / 28                                & \textbf{15} / 28                              & \textbf{15} / 28                          & \textbf{15} / 28                            & \textbf{15} / 28                                 \\ \hline
        \end{tabular}
        \label{tab:global_performance}
\end{table*}

\todo{Table~\ref{tab:global_performance} presents the results of the comparison with the baselines. Our proposed planner outperforms the.. }
\begin{table}[b]
        \caption{Statistics for the different motion planning strategies for static collision avoidance. MPCC: Model Predictive Contour Control; MPC: Tracking MPC; DW: Dynamic Window.}
        \centering
        \begin{tabular}{|p{1.34cm}|p{0.9cm}|p{0.54cm}|p{0.54cm}|p{0.54cm}|p{0.54cm}|p{1.12cm}|}
                \hline
                \multirow{2}{1.34cm}{Coordination strategies} & \multirow{2}{0.9cm}{Arrival time (s)} & \multicolumn{4}{c|}{Trajectory length (m)} & \multirow{2}{1.12cm}{Av.comp. time (ms)} \\ \cline{3-6}
                                                         &                                & min.      & max.     & av.      & std      &                                 \\ \hline
                MPCC                                       & 0.56                           & 4.82      & 7.09     & 5.72     & 0.89     & 15.2                               \\ \hline
                MPC                                       & 0.70                           & 4.31      & 4.54     & 4.43     & 0.09     & 115.3                               \\ \hline
                DW                                       & 0.70                              & 4.18         & 4.80        & 4.51        & 0.24        & 16.2                               \\ \hline
        \end{tabular}
        \label{tab:global_performance}
\end{table}

\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\# agents} & \multicolumn{3}{c|}{Clearance (m) (Mean / 99th percentile)} & \multicolumn{3}{c|}{\% failures (\% collisions / \% stuck)} & \multicolumn{3}{c|}{Traveled distance (m) (Mean / Std.)} \\ \hline
\multicolumn{2}{|c|}{}        & DW                & CADRL               & LMPCC               & DW               & CADRL               & LMPCC              & DW              & CADRL             & LMPCC             \\ \hline
\multicolumn{2}{|c|}{2}                &   1.10 / 0.63                &      0.75  / 0.63            &   0.97 / 0.65                  &  31.0 (30.0 / 1.0)                & 47.0 (45.0 / 3.0)                  &  \textbf{2.0 (0.0 / 2.0)  }                &    17.99  / 3.89           &     19.27 / 3.7              &     \textbf{15.8 / 3.23    }          \\ \hline
\multicolumn{2}{|c|}{4}                &        0.68 / 0.63           &      0.67/0.63                &     0.88 / 0.633                &  74.0 (71.0 / 3.0)                &  79.0 (76.0 / 3.0)                 &  \textbf{5.0 (2.0 / 3.0)  }                &     19.5 /5.28            &      21.34 / 4.4             &      \textbf{ 15.77 / 4.55 }           \\ \hline
\end{tabular}
 \label{tab:global_performance}
\end{table*}

==> sec/method_backup.tex <==
\section{METHOD}\label{sec:method}
% Clothoidal spline \cite{walton1990clothoidal}
The goal of the \ac{lmpcc} is to generate feasible and optimal motion with respect to the defined cost along the constructed local reference path. The \ac{lmpcc} framework contains the following contributions:
\begin{enumerate}
\item The use of a transition function between waypoints to eliminate the non-differentiable representation of the reference path (\cref{sec:reference_path}).
\item The application of a search routine to solve the approximation of the path progress estimation (\cref{sec:path_parameter}).
\item Static obstacle avoidance by explicitly constraining the control problem to an approximation of the collision-free area (\cref{sec:static_collision}).
\item A bound on the Minkowski sum of a circle and an ellipse for moving obstacles (\cref{sec:collision_avoidance2}).
\end{enumerate}
\subsection{Global planning / Generation of reference path}\label{sec:reference_path}
Given a goal position $\boldsymbol{p}_{\text{goal}}$, first, we use a global planning method (such as RRT \cite{kuffner2000rrt}) to compute a collision-free path through the static environment representation from an initial position $\boldsymbol{p}_0$. This global reference path $\pazocal{P}$ consists of $M$ points defined as $\boldsymbol{p}_m = [x^p_m,y^p_m] \in \W$ with $m \in \pazocal{M} := \{1,\dots,M\}$. Then, we split the path into segments delimited by $[x^p_m,y^p_m]$ and $[x^p_{m+1},y^p_{m+1}]$. We use cubic spline interpolation to obtain an analytical expression of the reference path for each segment, connecting each of the global reference path points with a polynomial of length $s_m$. The efficient implementation of \cite{tkspline} allows splines to be generated in $\order(q)$ and evaluation of the spline at a single point to be performed in $\order(\log (q))$, where $q$ is the number of input data points. This efficiency motivates our choice of local spline fitting during execution. Hence, we define the piece-wise spline segments as a function of the traveled distance along the reference path $\theta$. This path parameter equals zero at the start of each path segment and continuously increases along the segment. \cref{fig:mpcc_path} shows three reference path segments and the projected robot position on the reference path. 
\begin{figure}[t]
\centering
\includegraphics[trim={0cm 0 0cm 0cm},clip,width=0.8\columnwidth]{images/mpcc_path.pdf}
\caption{Reference path representation}
\label{fig:mpcc_path}
\end{figure}
Each path segment is composed of the interpolated reference trajectory points concatenated with a corresponding velocity reference, that is, $\boldsymbol{R}_m := [\boldsymbol{p}_m^{r^\textrm{T}},v_{\textrm{ref},m}]^\textrm{T}$. This velocity reference depends on the environment and should be provided by the route planning module. The cubic polynomials that define the local reference points $\boldsymbol{p}^r$ are a function of $\theta$ and are given by:
\begin{equation}\label{eq:analytic_reference_path}
\boldsymbol{p}^r_m(\theta)\! =\!
\begin{bmatrix}
x^r_m\\
y^r_m
\end{bmatrix}\! =\! \begin{bmatrix}
a^x_{m,1}\theta^3 + a^x_{m,2}\theta^2 + a^x_{m,3}\theta  + a^x_{m,4} \\
a^y_{m,1}\theta^3 + a^y_{m,2}\theta^2 + a^y_{m,3}\theta  + a^y_{m,4}
\end{bmatrix}
\end{equation}
where $[a^x_{m,1}, \dots, a^x_{m,4}]$ and $[a^y_{m,1},\dots, a^y_{m,4}]$ are the coefficients of the cubic polynomials at segment $m$ of both splines. \looseness=-1

We consider a limited set of path segments $\boldsymbol{R}_m \subset \pazocal{R}$ of the reference path. This allows to reduce the computational complexity of the planning problem and allows segments outside of the local reference path to change over time. We define the local reference path $\boldsymbol{L}^r$ at current time by linking $\eta$ path segments, starting from the $m$-th closest path segment, that is,
\begin{equation}\label{eq:L_m}
    \boldsymbol{L}^r = \{ R_i \in \pazocal{R} | i = [ m, \dots, m + \eta] \}
\end{equation}
%An analytical expression of the derivative of the local reference trajectory is given by
%\begin{align}
%\begin{split}
%\dot{x}^r_m = f_m^x(\theta)\sp{\prime} = 3a^x_1\theta^2 + 2a^x_2\theta + a^x_3\\
%\dot{y}^r_m = f_m^y(\theta)\sp{\prime}  = 3a^y_1\theta^2 + 2a^y_2\theta + a^y_3
%\end{split}
%\end{align}

\subsection{Selecting the number of path segments}
We provide a strategy to select $\eta$ to guarantee that the local reference path representation captures enough information of the global path to be tracked by the \ac{lmpcc}. In particular, we provide a strategy to select the length of the local reference path with respect to the prediction horizon. The number of path segments $\eta$ to be included in the local reference path is a function of the prediction horizon length, the individual path segment lengths, and the speed of the \ac{agv} at each time instance, as described below:
\begin{equation}\label{eq:eta}
\underbrace{\sum^{m + \eta}_{i = m} s_i}_{\text{Local reference path length}} \geq \underbrace{\tau \sum^{N}_{j = 0} v_{j}}_{\text{Traveled distance in horizon}}    ,
\end{equation}
where $\tau$ is the length of the discretization steps along the horizon.
We use an upper bound on~\eqref{eq:eta} by considering maximum longitudinal velocity $v_{\max}$ and select $\eta$ such that

% $\sum^{m + \eta}_{i = m} s_i \geq T_{\textrm{horizon}} \cdot v_{\max}$.

\begin{equation}\label{eq:eta_upper}
\sum^{m + \eta}_{i = m} s_i \geq T_{\textrm{horizon}} \cdot v_{\max}
\end{equation}
\subsection{Progress on reference path}\label{sec:path_parameter}
\ac{mpcc} keeps track of the path progress along the total reference path using the path parameter $\theta$. Finding the corresponding path parameter, however, involves solving another optimization problem which would increase the computational cost of the algorithm \cite{schwarting2017safe}. 
If the distance between waypoints is small in relation to their curvature, spline parametrization can be regarded as reasonable approximations of arc-length parametrizations. Therefore, conventional \ac{mpcc} assumes that the evolution of path parameter can be approximated by the traveled distance of the robot:
\begin{equation}\label{eq:path_variable}
\theta_{k+1} \approx \theta_k + v_k \tau
\end{equation}
where $v$ is the forward velocity of the controlled vehicle. The estimation of the path parameter, however, has shown to be quite coarse, especially when the AGV must deviate from the reference path during an avoidance maneuver. During such a maneuver, the path parameter starts drifting. \ac{lmpcc} resolves the problem of the drifting path parameter by performing line search around the estimated path parameter, as  Algorithm \ref{alg_theta} describes, resulting in the refined path variable estimation $\tilde{\theta}$. In particular, note that the evolution of the path variable in the prediction horizon still matches \cref{eq:path_variable}, while the initialization of the path parameter is done with the refined approximation $\tilde{\theta}_0$ at each iteration. 

\begin{algorithm}
\caption{Refined path variable estimation}\label{alg_theta}
\begin{algorithmic}[1]
\State {$\theta_0 = \theta_{previous} + v_k\tau$}
\State {$\text{window}= [\theta_0 - L_{\text{window}} : \theta_0 + L_{\text{window}}]$}
% \State $\textbf{int} \text{ N}_{\text{sample}}$
% \State $\textbf{double} \text{ window }$
\For {$\text{each } \theta_{\text{sample}} \text{ in window}$}
\State {$\text{Compute distance to } \theta_{\text{sample}}$}
\If {$\text{distance} < \text{distance}_{\text{min}}$}
\State {$\text{distance}_{\text{min}} = \text{distance}$}
\State {$\tilde{\theta}_0 = \theta_{\text{sample}}$}
\EndIf 
\EndFor
\end{algorithmic}
\end{algorithm}
\subsection{Maintaining continuity over the local reference path}
To concatenate the properties of separate reference path segments into the local reference path $\boldsymbol{L}^r$ that is tracked by the \ac{lmpcc}, we provide a differentiable expression of the corresponding parameters over the prediction horizon. We use a sigmoid activation function $\sigma$ to link $\eta$ path segments $\boldsymbol{R}_m$ as in \cref{eq:L_m}. In order to connect the analytical expressions of the reference path segments (\cref{eq:analytic_reference_path}), we multiply the piece-wise spline sections by their corresponding activation function $\sigma_m(\theta,s_m)$, as follows:
\begin{equation}\label{eq:concatenation}
    \bar{\boldsymbol{L}}^r(\theta) = \sum^{m+\eta}_{i = m} [   \bar{\boldsymbol{p}}^r(\theta_k)^\textrm{T}, \bar{v}_{ref}]^\textrm{T} \cdot \sigma_m(\theta,s_m)
\end{equation}
% \begin{align}\label{eq:concatenation}
% \begin{split}
%     L_k(\theta) &= \begin{bmatrix}
%     x^r(\theta)\\
%     y^r(\theta)\\
%     v^r(\theta)
%     \end{bmatrix} = \\
%     &= \sum^{m + \eta}_{i = m} \Bigg( \sigma_i(\theta,s_m) 
%     \cdot \prod_{j = m}^{i - 1}(1 - \sigma_i(\theta,s_m))
%     \begin{bmatrix}
%     x^r_i \\
%     y^r_i \\
%     v^r_i
%     \end{bmatrix}
%     \Bigg)
% \end{split}
% \end{align}

\subsection{Static Collision avoidance}\label{sec:static_collision_avoidance}
Figure \ref{fig:obstacles} provides and overview of our collision avoidance strategy that we discuss in more details below. The AGV is represented by $n_{\text{disc}}$ discs centered in $\boldsymbol{p}_j^B$, where $\boldsymbol{p}_j^B$ is the position on the $j$-th disc in the AGV body-frame and $n_{\textrm{disc}}$ is the number of discs used to bound the AGV, $j\in\pazocal{J}^{\textrm{disc}}:=\{1,2,\ldots,n_{\textrm{disc}}\}$.

\begin{figure}[h!]
\centering
\includegraphics[trim={0cm 0cm 0cm 7cm},clip ,width=\columnwidth]{images/polygon_vis.pdf}
\caption{Overview of our collision avoidance strategy.}
\label{fig:obstacles}
\end{figure}
%\subsubsection{Position constraints on static obstacles}\label{sec:static_collision}
It is assumed that the reference path is free of static obstacles. When the \ac{agv} deviates from the reference path, it should be guaranteed that static obstacles are avoided. Figure~\ref{fig:obstacles} shows how we approximate a collision-free region along the prediction horizon. In particular, we use the shifted optimal state sequence computed at the previous time instance $t-1$, namely, $\boldsymbol{z}^*_{1:N|t-1}$. Then, the $N$-th element to append to $\boldsymbol{z}^*_{1:N|t-1}$ is obtained by extrapolating from the last element of $\boldsymbol{z}^*_{1:N|t-1}$. The resulting vector is $\boldsymbol{\bar z}^*_{1:N|t-1}$. This sequence of states $\boldsymbol{\bar z}^*_{1:N|t-1}$ is used to center the circles depicted in Figure~\ref{fig:obstacles}. The collision-free region is then computed as follows. The radii are found by expanding each circle in the occupancy grid map of the environment until an occupied cell is detected. The radius of the collision free circle is denoted by $r_k$. The approximated collision free area is introduced as an inequality constraint on the current \ac{agv} position such that $\B(\boldsymbol{z}_k) \cup \pazocal{O}^{\textrm{static}} =\emptyset\,\forall\, k\in \{0,\dots,N\}$.

Given $\boldsymbol{\bar z}^*_{1:N|t-1}$, we enforce that the distance of the \ac{agv} with respect to these positions must be smaller than a circle with radius $\bar {r}_{k,j} := r_k - r_\textrm{disc} - \|\boldsymbol{p}_j^B\|_2^2$  $\forall k\in\{0,\dots,N\}$:
\begin{align}\label{eq:env_constraint}
\begin{split}
    c_{k}^{\textrm{env},j}\!(\boldsymbol{z}_k)\! = \bar {r}_{k,j} -  \|\boldsymbol{\bar p}^*_{k|t-1} - \boldsymbol{ p}_k\|_2^2 &\Big\rvert_{k,j} > 0
\end{split}
\end{align}

\subsection{Dynamic collision avoidance}\label{sec:dynamic_collision_avoidance}
Recall that each moving obstacle $A_i$ is represented by state $\boldsymbol{z}^{A_i}(t)$, and ellipse dimensions $a$ and $b$. The collision avoidance constraints can now be defined as an inequality constraint for each $j$-th disc bounding the robot with respect to the distance of each obstacle $i \in \{1,\dots,n\}$ at time k as depicted in \cref{fig:obstacles}. Omitting $i$ for simplicity, the inequality constraint on each disc of the \ac{agv} with respect to the obstacles is given by:
\begin{equation}\label{eq:ineq_constraint}
\begin{split}
\!\!\!c_k^{\textrm{obst},j}(\boldsymbol{z}_k) \!\!= \!\!\begin{bmatrix}
\Delta x_k^j\\
\Delta y_k^j
\end{bmatrix}^\textrm{T}\!\!\!\!
R(\psi)^\textrm{T}\!\!\begin{bmatrix}
\frac{1}{\alpha^2} & 0\\ 0 & \frac{1}{\beta^2}
\end{bmatrix}\!\! R(\psi)\!\!\!\ \begin{bmatrix}
\Delta x_k^j\\
\Delta y_k^j
\end{bmatrix}&\Bigg\rvert_{k,j} \!\!\!\!> 1
\end{split}
\end{equation}
The distance from disc $j$ to the obstacle is split into its $\Delta x^j$ and $\Delta y^j$ components as shown in \cref{fig:obstacles}. $R(\psi_k)$ is the rotation matrix corresponding to the heading of the obstacle and $\alpha$ and $\beta$ are the resulting axes of the ellipse constraint.

\begin{figure}[h!]
\centering
\includegraphics[trim={0cm 0cm 0cm 0cm},clip ,width=\columnwidth]{images/lambda.pdf}
\caption{Exact safety boundary computation}
\label{fig:bound}
\end{figure}

It is important to notice that previous approaches assumed that the Minkowski sum of an ellipse with a circle is an ellipsoid with semi-major $\alpha = a + r_{\text{disc}}$ and semi-minor axis $\beta = b + r_{\text{disc}}$ \cite{schwarting2017safe}. This assumption, however, is not correct and collision can still occur \cite{chen2017constrained} as represented in Fig. \ref{fig:bound} with the grey ellipsoid as the considered bound and in black the actual Minkowski sum. 
In this section we present what are the exact values for $\alpha$ and $\beta$ such that collision avoidance is guaranteed, represented by the orange ellipsoid.
% According with the theorem proposed by \cite{uteshev2015metric} the minimum distance between two quadratic shapes is the minimal positive zero of the polynomial:

\begin{lem}\label{eq:minimum_polynom}
        Let $X^TE_1X=1$ and $X^TE_2X=1$ be two quadratics in $\mathrm{R}^n$. Iff the matrix $E_1-E_{2}$ is sign definite then the square of the distance between the ellipsoid $X^TA_1X=1$ and the quadratic $X^TA_2X=1$ equals the minimal positive zero of the polynomial.
        \begin{align*}
                 F(z) = D_\lambda(\det{\lambda*E_1+(z-\lambda E_2)-\lambda(z-\lambda E_1E_2)})
        \end{align*}
        where $D$ stands for the discriminant of the polynomial treated w.r.t. $\lambda$ \cite{uteshev2015metric}.
\end{lem}

%We use a determinantal representation of the discriminant as defined in \cite{uteshev2015metric}. 
The minimum distance equation can be used to compute the minimum dimensions of an ellipsoid which correctly bounds the Minkowski Sum. Consider two ellipsoids $E_1= Diag(\frac{1}{(a)^2}\frac{1}{(b)^2})$ with semi-major axis $a$ and semi-minor axis $b$ and $E_2 = Diag(\frac{1}{(a+\delta)^2}, \frac{1}{(b+\delta)^2})$. $E_2$ representing the ellipsoid $E_1$  enlarged by $\delta$.
The \cref{eq:minimum_polynom} can now be used to obtain the minimum distance between $E_1$ and $E_2$ resulting in the following equation:

\begin{equation}
    Dist_{min}=\frac{4 a b \delta^2 + 2 a \delta^3 + 2 b \delta^3}{a^2 + 2 a b + b^2 + 2 a \delta + 2 b \delta}
\end{equation}

In order to find the correct bounding ellipsoid it is necessary to find the value of $\delta$ such that $Dist_{min} \ge r_{disc}$. Since the distance equals the minimal positive zero of the polynomials the solution can be found numerically in the positive neighborhood of zero. A close formula can also be obtained but due to its length it is not presented in this paper. The resulting bounding ellipse and shape of the Minkowski Sum can be observed in \cref{fig:bound}


In order to ensure collision-free motions the radius is enlarged by a factor $\lambda$: 
\begin{equation}
\begin{bmatrix}
\alpha\\
\beta
\end{bmatrix} = \begin{bmatrix}
a + \lambda r_{\text{disc}}\\
b + \lambda r_{\text{disc}}
\end{bmatrix}_{'}
\end{equation}
where $\lambda$ is computed such that the curvature of the constraint ellipsoid is a lower bound of the curvature of the Minkowski sum, as follows:
\begin{equation}\label{eq:new_bound}
    \lambda = \min\left[\begin{split}{\frac{(a^2 + b r)(1-\frac{2 a b}{a^2 + b r} + \sqrt{
   \frac{(a-2b)^2+b r)}{a^2 + b r})}}{2 b}}\\
   {\frac{(b^2 + a r)(1 -\frac{2 a b}{b^2 + a r} + \sqrt{\frac{(-2a+b)^2+a r}{b^2 + a r})}}{2 a}}
   \end{split}\right]
\end{equation}
This guarantees that the constraint ellipsoid entirely bounds the collision space.
% euqation for delta offset instead of lambda factor
%\begin{equation}\label{eq:new_bound}
    %\lambda = \min\left[\begin{split}{\frac{(a^2 + b r)(1-\frac{2 b(a+r)}{a^2 + %b r} + \sqrt{1+4
   %\frac{b^2-ab}{a^2 + b r})}}{2 b}}\\
   %{\frac{(b^2 + a r)(1 -\frac{2 a(b+r)}{b^2 + a r} + \sqrt{1+4\frac{b^2-a %b}{b^2 + ar})}}{2 a}}
%   \end{split}\right]
%\end{equation}
\subsubsection{Repulsion from dynamic obstacles}\label{sec:collision_avoidance3}
A penalty in the cost function that resembles repulsion from dynamic obstacles ensures clearance between the \ac{agv} and the obstacles. The penalty is defined as follows:
\begin{equation}\label{eq:repulsive}
J_{\text{repulsive}}(\boldsymbol{z}_k) = Q_R \sum^{n}_{i = 1} \bigg( \frac{1}{(\Delta x_k)^2 + (\Delta y_k)^2 + \gamma} \bigg) \quad \!,
\end{equation}
 where $Q_R$ is the weight on the repulsive forces \cite{Abbas2017}. The distance from the \ac{agv} to the dynamic obstacles is given in its separate $\Delta x_k$ and $\Delta y_k$ components as in \cref{fig:obstacles}. A small value $\gamma$ is introduced to avoid a division by zero, for numerical stability of the solver~\cite{Houska2011a}.
\subsection{Local Model Predictive Contouring Control} 
As introduced in \cref{sec:reference_path}, the global reference path $\pazocal{P}$ consists of $M$ segments, resulting in a local reference trajectory $\bar{\boldsymbol{L}}^r(\theta_k)$ with $\eta$ segments, starting from the $m$-th closest path segment. The local contour error $\epsilon^c$ and the longitudinal error $\epsilon^l$ are expressed as a function of $\theta$ as visualized in \cref{fig:mpcc}. 
\begin{figure}[t]
\centering
% \includegraphics[trim={11.5cm 0 1.8cm 14.5cm},clip,width=\columnwidth]{images/MPCC_robotframe.pdf}
\includegraphics[trim={11.5cm 0 1.8cm 14.5cm},clip,width=\columnwidth]{images/MPCC_worldframe.pdf}
\caption{Approximated contour and lag error on the path segment.}
\label{fig:mpcc}
\end{figure}
With $\bar{\boldsymbol{p}}^r(\theta_k)$ being the local reference path points, the contouring and longitudinal error vector $\boldsymbol{e}_k := [\tilde{\epsilon}^c(\boldsymbol{z}_k,\theta_k),\tilde{\epsilon}^l(\boldsymbol{z}_k,\theta_k)]^\textrm{T}$ is defined as follows:
\begin{align}
\boldsymbol{e}_k = 
\begin{bmatrix}
\sin \phi(\theta_k)& -\cos \phi(\theta_k)\\
- \cos \phi(\theta_k)&-\sin \phi(\theta_k)
\end{bmatrix}
\big( \boldsymbol{p}_k - \bar{\boldsymbol{p}}^r(\theta_k) \big).
\end{align}

% \begin{align}\label{eq:errors}
% \begin{split}
% \hat{\epsilon}^c(\boldsymbol{z}_k,\theta_k) &= \sin \phi(\theta_k) \big( x_k - x^r(\theta_k)\big) - \cos \phi(\theta_k) \big( y_k - y^r(\theta_k)\big)\\
% \hat{\epsilon}^l(\boldsymbol{z}_k,\theta_k) &= -\cos \phi(\theta_k) \big( x_k - x^r(\theta_k)\big) - \sin \phi(\theta_k) \big( y_k - y^r(\theta_k)\big)
% \end{split}
% \end{align}

%The path parameter allows the definition of two types of errors that can be included in the cost function to enforce that the \ac{agv} tracks the reference path. Ideally, the contour error, $\epsilon^c$, and the longitudinal error, $\epsilon^l$, would be expressed using the closest point to the local reference path as in \cref{fig:mpcc}.
In order to ensure progress along the reference path, the conventional MPCC scheme proposes to add a negative cost term proportional to the travelled distance. In contrast, we introduce a cost term that penalizes the deviation of the vehicle velocity $v_k$ with respect to a reference velocity $v_{\textrm{ref}}$. The reference velocity is provided according to \cref{eq:concatenation}, allowing the vehicle to adapt its speed according to the path segment that it is tracking. Now, the LMPCC tracking cost is defined as
$J_{\text{tracking}}(\boldsymbol{z}_k,\theta_k) = \boldsymbol{e}_k^TQ_{\epsilon}\boldsymbol{e}_k + Q_v(v_{ref} - v_k)^2$,
% where $Q_{\epsilon}$ and $Q_v$ are the weights on the path error and the reference velocity, respectively.
Additionally, the cost function also penalizes with weight $Q_u$ the inputs, that is, $J_{\text{input}}(\boldsymbol{z}_k,\theta_k) = \boldsymbol{u}_k^TQ_{u}\boldsymbol{u}_k$.
We can now formulate our \ac{lmpcc} control problem:
\begin{align}\label{eq:control_problem}
\begin{split}
J^* = &\min_{\boldsymbol{z}_{0:N},\boldsymbol{u}_{0:N-1}} \sum^{N-1}_{k =0} J(\mathbf z_k,\mathbf u_k, \theta_k) + J(\boldsymbol{z}_N,\theta_N) \\
\text{s.t.} \quad & \boldsymbol{z}_{k+1} := f(\boldsymbol{z}_{k},\boldsymbol{u}_{k}),  \\
& \theta_{k+1} = \theta_{k} + v_{k} \tau,  \\
& \boldsymbol{z}_{\min} \leq \boldsymbol{z}_k \leq \boldsymbol{z}_{\max},  \\
& \boldsymbol{u}_{\min} \leq \boldsymbol{u}_k \leq \boldsymbol{u}_{\max}, \\
& c_k^{\textrm{env}}(\boldsymbol{z}_k) > 0, \qquad \quad  \\
& c_k^{\textrm{obst},j}(\boldsymbol{z}_k) > 1, \quad \forall j,\, \forall \textrm{obst}\\
& \mathbf{z}_0 = z_{\textrm{init}}, \, \theta_0 = \tilde{\theta}  \\
\end{split}
\end{align}
where $ J(\mathbf z_k,\mathbf u_k, \theta_k): = J_{\text{tracking}}(\boldsymbol{z}_k,\theta_k)\! +\! J_{\text{repulsive}}(\boldsymbol{z}_k) \!+\! J_{\text{input}}(\boldsymbol{u}_k)$. \cref{alg_lmpcc} summarizes our design. Each control iteration, feedback steps are performed until either a \ac{kkt} condition \cite{kuhn1951} or the maximum number of iterations is satisfied (line ~\ref{alg:kkt}).

\begin{algorithm}
\caption{Local Model Predictive Control}\label{alg_lmpcc}
\begin{algorithmic}[1]
\State Given $z_0$, $z_{\textrm{goal}}$, $\pazocal{O}^{\textrm{static}}$, $\pazocal{O}_ k^{\textrm{dyn}}$, and $N$
\State {\textbf{Initialization}: $k = 0$}
    \State Build global path $\pazocal{P}$ \cref{eq:analytic_reference_path,eq:concatenation}
    \State Select $\eta$ according to \cref{eq:eta_upper}
    \State Build $\bar{\boldsymbol{L}}^r(\theta_k)$ according to  \cref{eq:analytic_reference_path,eq:concatenation}
\While{$\boldsymbol{z}_k \ne \boldsymbol{z}_{\textrm{goal}}$ in parallel}
    \State Process sensor data
    \State Estimate $\tilde{\theta}_0$ according to \cref{alg_theta}
    % \State Lock $\bar{\boldsymbol{L}}^r(\theta)$
    \State $\text{Compute }r_k \text{ along } \boldsymbol{\bar z}^*_{1:N|t-1}$
    \While{\texttt{iter} $< \textrm{\texttt{iter}}_{\max} \wedge \textrm{KKT} > \textrm{threshold}$} \label{alg:kkt}
            \State Solve \cref{eq:control_problem}
            \State $\texttt{iter}=\texttt{iter}+1$
    \EndWhile
    \State$\text{Apply } \boldsymbol{u^*_0}$
    \If{$\theta_k>s_k$}
        \State $k=k+1$
        \State Re-plan global path $\pazocal{P} \setminus \boldsymbol{p}^r$ 
        \State Build $\bar{\boldsymbol{L}}^r(\theta_k)$ according to  \cref{eq:analytic_reference_path,eq:concatenation}
    \EndIf 
\EndWhile
\end{algorithmic}
\end{algorithm}

% \begin{algorithm}
% \caption{Local Model Predictive Control}\label{alg_lmpcc}
% \begin{algorithmic}[1]
% \State Given $z_0$, $z_{\textrm{goal}}$, $\pazocal{O}^{\textrm{static}}$, $\pazocal{O}_ k^{\textrm{dyn}}$, and $N$
% \State {\textbf{Initialization}: $k = 0$}
%     \State Build global path $\pazocal{P}$
%         \For{$m = 0,1,2, \ldots M-1$}
%             \State Build $\boldsymbol{R}_m$ according to \cref{eq:analytic_reference_path}
%         \EndFor 
%     \State Select $\eta$ according to \cref{eq:eta_upper}
% \While{$\boldsymbol{z}_k \ne \boldsymbol{z}_{\textrm{goal}}$ in parallel}
%     \State Process sensor data
%     \State Estimate $\tilde{\theta}_0$ according to \cref{alg_theta}
%     \State Lock $\bar{\boldsymbol{L}}^r(\theta)$
%     \For{$m \ne k \in $range($M$)}
%         \State Re-plan global path: $\boldsymbol{R}_m$ 
%         \State Build $\overline{R}$: polynomial fitting: $\boldsymbol{R}_m$
%     \EndFor 
%     \State $\text{Compute }r_k \text{ along } \boldsymbol{\bar z}^*_{1:N|t-1}$
%     \While{\texttt{iter} $< \textrm{\texttt{iter}}_{\max} \wedge \textrm{KKT} > \textrm{threshold}$}
%             \State Solve \cref{eq:control_problem}
%             \State $\texttt{iter}=\texttt{iter}+1$
%     \EndWhile
%     \State$\text{Apply } \boldsymbol{u^*_0}$
%     \If{$\theta_k>s_k$}
%         \State $k=k+1$
%     \EndIf 
% \EndWhile
% \end{algorithmic}
% \end{algorithm}

==> sec/preliminaries_backup.tex <==
\section{PRELIMINARIES}\label{sec:problem_formulation}

\todo{Reviewer 4: The approach simply assumes that the future trajectory is known exactly.}

Let $B$ denote an AGV on the plane $\W = \mathbb{R}^2$. $B$ can be represented by the following discrete nonlinear system:
\begin{equation}\label{eq:state_dynamics}
\boldsymbol{z}(t+1) = f(\boldsymbol{z}(t),\boldsymbol{u}(t)),
\end{equation}
where $\boldsymbol{z}(t)$ and $\boldsymbol{u}(t)$ represent the state and the command at time $t\geq 0$ \footnote{In the remainder of the paper we omit the time dependency when it is clear from the context.}, respectively. % For a mobile robot, for example, the state is $\boldsymbol{z} := [\boldsymbol{p}, \phi]$, where $\boldsymbol{p}$ is the position on the ($x$,$y$) plane and $\psi$ is the heading angle. 
The configuration of the AGV is denoted in configuration space $\pazocal{C} = \mathbb{R}^2 \times \pazocal{S}$ by $\boldsymbol{z}(t) \in \pazocal{C}$.
The area occupied by the \ac{agv} at state $\boldsymbol{z}$ is $\pazocal{B}(\boldsymbol{z})$. $\pazocal{B}(\boldsymbol{z})$ is approximated by a union of circles, that is, $\pazocal{B}(\boldsymbol{z}) \subseteq \bigcup_{c \in \{1,\dots,n_c \}} \pazocal{B}_c(\boldsymbol{z}) \subset \W$, where $n_c$ is the number of circles. \looseness=-1

We consider static and dynamic obstacles. In particular, the static obstacle environment is assumed to be captured in an occupancy grid map. The area occupied by the static obstacles is $\pazocal{O}^{\textrm{static}} \subset \pazocal{W}$. Furthermore, each moving obstacle $A_i$ is represented by an ellipse of area $\A_ i$. Consider a set of moving obstacles $A_i$ with $i \in \pazocal{I} := \{1, \dots , n\}$ in $\W$, where $n$ can vary over time. The area occupied by all moving obstacles at time instant $t$ is given by $\pazocal{O}_t^{\textrm{dyn}} = \bigcup_{i \in \{1,\dots,n \}} \A_i(\boldsymbol{z}_i(t))$, where $\boldsymbol{z}_i(t)$ denotes the state of $A_i$ at time $t$. The size of an ellipsoid associated with the obstacle is defined by $a$ and $b$, the semi-major and semi-minor axes of the ellipse, respectively.

The objective is to generate collision free motion for $B$ through $\W$, from its current state to a desired end configuration. This can be formulated as an optimization problem as follows:
\begin{subequations}
\begin{align}
J^* = & \min_{\boldsymbol{z}_{0:N},\boldsymbol{u}_{0:N-1}} \sum^{N-1}_{k =0} J(\boldsymbol{z}_k, \boldsymbol{u}_k, \theta_k) + J(\boldsymbol{z}_N,\theta_N)\\
\text{s.t.} \quad & \boldsymbol{z}_{k+1} = f(\boldsymbol{z}_{k},\boldsymbol{u}_{k}), \\
& \B(\boldsymbol{z}_k) \cap \big( \pazocal{O}^{\textrm{static}} \cup \pazocal{O}_k^{\textrm{dyn}} \big) = \emptyset,\\
% & \B(\boldsymbol{z}_k) \cap \pazocal{O}_{static} = \not \hspace{-0.05cm} 0\\
% & \B(\boldsymbol{z}_k) \cap \pazocal{O}_{dyn} = \not \hspace{-0.05cm} 0\\
& \boldsymbol{u}_k \in \U, \,\, \boldsymbol{z}_{k} \in \pazocal{X}\,.
\end{align}
\end{subequations}
where $\pazocal{X}$ and $\U$ are the set of admissible states and inputs, respectively. $\boldsymbol{z}_{1:N}$, $\boldsymbol{u}_{0:N-1}$ are the predicted state and control, respectively over a prediction horizon $T_{\textrm{horizon}}$ divided into $N$ prediction steps. $\theta_k$ denotes the predicted progress along the reference path. $J$ is a cost function defining the planner objectives. By solving the optimization problem above, we can obtain the optimal sequence of commands $\boldsymbol{u}^*_{0:N - 1}$ to guide the \ac{agv} along the reference path. 

In the remainder of the paper, we show how to formulate the objectives and how to define the collision avoidance constraints to track a local (generated) reference path in our LMPCC framework.
